Transverse Mode Control in Quantum Enhanced Interferometers: A Review and Recommendations for a New Generation

Adaptive optics has made significant advancement over the past decade, becoming the essential technology in a wide variety of applications, particularly in the realm of quantum optics. One key area of impact is gravitational-wave detection, where quantum correlations are distributed over kilometer-long distances by beams with hundreds of kilowatts of optical power. Decades of development were required to develop robust and stable techniques to sense mismatches between the Gaussian beams and the resonators, all while maintaining the quantum correlations. Here we summarize the crucial advancements in transverse mode control required for gravitational-wave detection. As we look towards the advanced designs of future detectors, we highlight key challenges and offer recommendations for the design of these instruments. We conclude the review with a discussion of the broader application of adaptive optics in quantum technologies: communication, computation, imaging and sensing.

==> mainmatter.tex <==
\section{Overview of  Gravitational Wave Detectors}
\subsection{Ring hEater}
\subsection{}

\section{Angular Alignment (may remove, depends on length)}
\subsection{Anderson Technique (and variants)}
\subsection{Ward Technique (and variants)}
\subsection{Novel Approaches}

\section{Beam to Resonator}
\subsection{Hartmann Cameras in aLIGO}
\subsection{Bulls Eye}
\subsection{Mode Converter}
\subsection{RF Beam Modulation}

\section{Beam to Beam}
\subsection{Coherent Beam Combination}
\subsection{RF Beam Modulation}

\section{Coupled Cavities}
\section{Alignment in aLIGO}


==> planning.tex <==
\section{Gravitational Wave Detectors}
\begin{planningbox}
    \begin{itemize}
        \item Assigned to: 
        \item Status: Not written
    \end{itemize}\
    Planned content: This should summarise the topology of interferometric gravitational wave detectors and introduce the importance of mode matching in these systems.
\end{planningbox}


\subsection{Angular Alignment}
\begin{planningbox}
    \begin{itemize}
        \item Assigned to: 
        \item Status: Not written
    \end{itemize}\
    Planned content: Discuss why angular alignment is important in suspended cavities.
\end{planningbox}

\subsection{Mode Matching on the Output Path}
\begin{planningbox}
    \begin{itemize}
        \item Assigned to: 
        \item Status: Not written
    \end{itemize}\
    Planned content: This should discuss, in detail, why mode matching on the output match is important.
\end{planningbox}

\subsection{Mode Matching of the Squeezer Beam}
\begin{planningbox}
    \begin{itemize}
        \item Assigned to: 
        \item Status: Not written
    \end{itemize}\
    Planned content: This should discuss, in detail, why mode matching on the output match is important.
\end{planningbox}

\subsection{Mode Matching in the Core Interferometer}
\begin{planningbox}
    \begin{itemize}
        \item Assigned to: 
        \item Status: Not written
    \end{itemize}\
    Planned content: Summarize why mode matching in the core IFO is important. I suggest breaking this section into two distinct sub-subsections: Thermal abberations and DC mode matching.
\end{planningbox}

\subsection{Point Defects}
\begin{planningbox}
    \begin{itemize}
        \item Assigned to: 
        \item Status: Not written
    \end{itemize}\
    Planned content: Discuss the effect of point defects on the mode structure in the cavity (possibly seek Daniel Brown's input).
\end{planningbox}

\subsection{Parametric Instability}
\begin{planningbox}
    \begin{itemize}
        \item Assigned to: 
        \item Status: Not written
    \end{itemize}\
    Planned content: Discuss what parametric instability is and why a mode sensor might help.
\end{planningbox}

\subsection{Higher Order Mode Carrier Beam}
\begin{planningbox}
    \begin{itemize}
        \item Assigned to: 
        \item Status: Not written
    \end{itemize}\
    Planned content: A brief note about why 3G detectors may shift to HG33 and what changes if they do.
\end{planningbox}

\subsection{Commissioning}
\begin{planningbox}
    \begin{itemize}
        \item Assigned to: 
        \item Status: Not written
    \end{itemize}\
    Planned content: A brief note about commissioning and why mode sensors help.
\end{planningbox}

\section{Sensing Technologies}
\begin{planningbox}
    \begin{itemize}
        \item Assigned to: 
        \item Status: Not written
    \end{itemize}\
    Planned content: A brief introduction. In each section below, summarise research in the area and then discuss what problems this might be effective in solving.
\end{planningbox}

\subsection{Phase Cameras}
\subsubsection{Scanning Pinhole}
\subsubsection{Optically Demodulated}
\subsubsection{Others}
\subsubsection{Extraction of the Modal Weights from Phase Camera Images}

\subsection{Wavefront Sensing}
\subsubsection{Hartmann Sensors}
\subsubsection{Anderson/Ward Autoalignment}
\subsubsection{Bulls-Eye Photodectectors}

\subsection{Hetrodyne Detection}
\subsubsection{Mode Converter}
\subsubsection{Differential wavefront sensing and control using radio-frequency optical demodulation}

\subsection{Direct Mode Decomposition}
\begin{planningbox}
    \begin{itemize}
        \item Assigned to: Aaron Jones
        \item Status: Not written
    \end{itemize}\
    Planned content: Briefly summarise the direct mode decomposition technologies
\end{planningbox}
\subsubsection{Meta-Surface}
\subsubsection{SLM}

\section{Conclusions }
\begin{planningbox}
    \begin{itemize}
        \item Assigned to: 
        \item Status: Not written
    \end{itemize}
    Planned content: Discuss the technologies in the context of the problems listed above. For each problem we should discuss what technologies help
\end{planningbox}


==> sensors.tex <==
\section{Sensing technologies}

\subsection{Phase Cameras}
\placeholder{We should mention here, or somewhere else, as motivation for these kinds of sensors (phase and optical lock-in camera) that the ability to spatial profile the laser beam in a single frequency component is especially relevant for the power recycling cavity which has a g parameter ~ 1 (at least the Virgo one is), and hence the HOMs resonate together in the recycling cavity. Moreover, the upper and lower sidebands can experience different spatial distortions, having a different mode content and leading to power imbalances between the two sidebands. This would be also relevant when talking about the use of mode decomposition.}

\subsubsection{Scanning Pinhole}

Frequency-resolving spatio-temporal wavefront sensors employing a scanning pinhole were developed with GW interferometers in mind and the necessity to assert the spatial overlap of the carrier field with each sideband \cite{Goda2004}. These devices, commonly known as phase cameras, can measure the amplitude and phase of the laser wavefront at any beat-frequency of interest. This ability to image independently each upper and lower sideband is of great use to GW detectors, as imbalances in the sidebands have been known to cause issues in the longitudinal locking of cavities \cite{KeikoRAM}. \placeholder{Not sure if this paragraph should go here or above, but I put it here since the first LIGO phase camera was a scanning pinhole, and I added that to the text.}

The first applications of these devices in the context of GW detectors were at Initial LIGO Livingston to measure the mode structure of the power recycling cavity \cite{modeStructLIGO} and at Initial LIGO Hanford for a design check of the output mode cleaner, where thermal effects were observed [,]. 

Later, with the requirements of the Thermal Compensation System of Advanced Virgo (AdV) in mind, the phase camera was updated and further developed at Nikhef []. This is the design currently installed at AdV which has been used before successfully in monitoring thermal effects [] and is currently being used in the commissioning efforts towards O4 for optical characterization of the interferometer.

A frequency-shifted reference beam is combined on a beam splitter with the test beam, creating a heterodyne signal for each carrier and upper and lower sidebands. The laser beam under test is scanned over a pinhole photodiode. A mirror mounted on a 2-axis piezo scanner is used to that end. At AdV, the scanner produces an Archimedean spiral in 2D with a total of 16384 points acquired by the photodiode, forming a 128x128 raw image. This combination allows for acquiring images with high spatial resolution due to the use of the scanner and high frequency selectivity due to the high bandwidth achieved by the single photodiode. Demodulation at each beat frequency allows the reconstruction of amplitude and phase images built from the combination of the I and Q quadratures.

\subsubsection{Optically Demodulated}



